Transformer-Powered Surrogates Close the ICF Simulation-Experiment Gap with Extremely Limited Data

Recent advances in machine learning, specifically transformer architecture, have led to significant advancements in commercial domains. These powerful models have demonstrated superior capability to learn complex relationships and often generalize better to new data and problems. This paper presents a novel transformer-powered approach for enhancing prediction accuracy in multi-modal output scenarios, where sparse experimental data is supplemented with simulation data. The proposed approach integrates transformer-based architecture with a novel graph-based hyper-parameter optimization technique. The resulting system not only effectively reduces simulation bias, but also achieves superior prediction accuracy compared to the prior method. We demonstrate the efficacy of our approach on inertial confinement fusion experiments, where only 10 shots of real-world data are available, as well as synthetic versions of these experiments.

==> 003-coverletter.tex <==
To:
Editor,
Machine Learning: Science and Technology

I am writing to submit our manuscript entitled "Transformer-Powered Surrogates Close the ICF Simulation-Experiment Gap with Extremely Limited Data" for consideration in Machine Learning: Science and Technology. This paper presents a foundational approach for transfer learning in scientific problem, that is specifically designed for enhancing prediction accuracy in scenarios where ``extremely sparse'' experimental data is supplemented with simulation data.

Our work marks a significant advancement in the field of scientific machine learning, and provides an AI-driven solution for effectively calibrating real-world experimental data. We demonstrate unprecedented adaptability and effectiveness in eliminating the simulation bias, thereby leading superior prediction accuracy (a nearly 40\% improvement over the state-of-the-art method). The transformative aspect of our research lies in its potential to address critical challenges in simulation-driven science, especially in contexts where experimental data is scarce and expensive to obtain. While we demonstrate the efficacy of our approach in inertial confinement fusion, where only a limited number of real-world data samples are available, our findings have broad implications for numerous scientific fields reliant on computational simulations.

Our research stands at the intersection of machine learning innovation and its practical, high-impact application in the physical sciences, offering insights and methodologies that can be leveraged across various domains. Hence, we believe that this manuscript is particularly suited for the diverse and interdisciplinary readership of Machine Learning: Science and Technology. 

Thank you for considering our work for publication. We are confident that our findings will contribute significantly to the field and resonate with the diverse audience of Machine Learning: Science and Technology.

Sincerely,
Matthew L. Olson
Lawrence Livermore National Laboratory






==> documentBody/zzoldanalysis_neighborhoodsize.tex <==

\subsection{Graph Neighborhood Size}
We present a series of experiments to analyze the effectiveness of our proposed graph-based smoothing approach for hyper-parameter optimization in few-shot learning. We compare our method with the baseline of no smoothing, where the optimal configuration is selected solely based on the validation error rates. Moreover, we investigate the impact of varying the neighborhood size on the performance of our method.

\paragraph{Experimental Setup}

We investigate the impact of varying the neighborhood size on the performance of our proposed graph-based smoothing approach for selecting the optimal hyper-parameter configuration. Specifically, we consider the following scenarios:

\begin{itemize}
\item \textbf{No Smoothing (Neighborhood Size 0)}: In this scenario, we do not apply any graph-based smoothing and simply choose the configuration with the lowest validation error rate $\arg\min_{i} V_i$.
\item \textbf{Smoothing with Neighborhood Size 1}: We apply our proposed graph-based smoothing using a neighborhood size of 1, where nodes are connected if their corresponding configurations differ in exactly one dimension by a single parameter step $\arg\min_{i} \tilde{V}_i$.
\item \textbf{Smoothing with Neighborhood Sizes 2 to 5}: In these scenarios, we apply our proposed graph-based smoothing while systematically increasing the neighborhood size from 2 to 5. Larger neighborhood sizes result in more connected nodes and potentially smoother error rate estimates.
\end{itemize}

Our objective is to determine the optimal neighborhood size that balances the exploitation of the graph structure and the preservation of the original validation error rates.

\subsection{Results and Discussion}
\wkw{Do you really need this subsection? Isn't it obvious that increasing the neighborhood size results in smoother validation error?}
Figure \ref{fig:graph_results} shows the performance of our method as we increase the neighborhood size, in terms of the smoothed error rate.

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{figs/neighboorhood_graph.png}
\caption{Smoothed error rate as a function of the neighborhood size. Increasing the neighborhood size leads to higher smoothed error rates.}
\label{fig:graph_results}
\end{figure}

As can be seen from the results, increasing the neighborhood size leads to a higher smoothed error rate. This observation suggests that using larger neighborhoods might cause over smoothing, resulting in suboptimal hyper-parameter configurations. To avoid this issue, we choose the smallest neighborhood size that provides a balance between exploiting the graph structure and preserving the original validation error rates.

Based on our analysis, we select the hyper-parameter configuration corresponding to the smallest neighborhood size, which results in the best performance on the held-out test set. This finding confirms the effectiveness of our proposed graph-based smoothing approach for hyper-parameter optimization in few-shot learning. By leveraging the local structure of the hyper-parameter space and considering the information from neighboring nodes, our method can effectively identify optimal hyper-parameter configurations and outperform the baseline of no smoothing.

==> documentBody/zzoldintro.tex <==
Machine Learning for scientific data applications has continued to grow in popularity, particularly with recent advancements in Deep Neural Networks. The development of sophisticated simulation tools has enabled researchers to explore complex phenomena and generate large amounts of simulated data. However, in many scientific and engineering domains, acquiring experimental data remains challenging due to cost and time constraints. 
Recent advancements have helped address this challenge by leveraging transfer learning, e.g., deep learning-based techniques have been employed in the Inertial Confinement Fusion (ICF) physics setting for designing models that improve the prediction of fusion shot results by leveraging simulation data \citep{kustowski2022suppressing}. In this work, we build upon these efforts with a new model and training scheme, a transformer-based deep neural network with masked auto-encoder pretraining \citep{vaswani2017attention,he2022masked}, to significantly improve prediction capabilities in the simulation-to-real few-shot transfer learning setting.

Simulations often suffer from inherent biases, which can consequently affect the performance of predictive models adversely \citep{schmidt2009distilling}. \shusen{how does it affect it, this may be a good place to talk about domain shift etc. We need to provide more background on the general problem} Traditional methods for addressing this issue are limited, as they typically focus on a single output modality such as scalar values representing physical quantities, and they fail to utilize the full potential of multi-modal data such as a combination of scalars and diagnostic images/videos. 
% \shusen{we may want to frame these differently as they will not be very understandable for domain reader}
Furthermore, in the context of few-shot learning, noisy validation error rates pose a significant challenge, often resulting in less generalizable hyper-parameter selection and undermining the effectiveness of traditional optimization approaches, e.g., grid search and random search \citep{bergstra2012random}.

To overcome these limitations, we propose a novel method that combines Transformer-based Masked Auto-Encoders (MAEs) with an innovative graph-based hyper-parameter optimization technique. MAEs efficiently capture the important correlations between different output modalities, as well as between simulation inputs and outputs \citep{he2022masked}.  Additionally, our approach to hyper-parameter optimization involves modeling hyper-parameters as a sparse graph to smooth validation set error rates, which significantly outperforms traditional minimum-validation-set-error-based methods.

We demonstrate the effectiveness of our method through extensive cross-validation, evaluated on real and synthetic ICF datasets. Our results indicate that the proposed approach systematically improves predictions, outperforming baseline methods and offering a promising solution for a wide range of problems that cannot be solved by incorporating physics-informed laws \citep{karniadakis2021physics}.

\shusen{I think this should be moved to the front as the context for motivating the work}
Our goal is to enhance the predictive capabilities of models operating on data collected from real ICF experiments, also known as \emph{shots}. These experiments are characterized by nine input parameters that describe the physical setup; ten output scalars, such as energy yield; and output x-ray emissions, which are formatted as images. Due to the high costs and time-consuming nature of setting up these experiments, the availability of real-world data points is severely limited. To address this dilemma, researchers often employ simulation software to generate additional data points, albeit at the cost of a million CPU hours for each three-dimensional simulation \citep{kustowski2022suppressing}. Nevertheless, \citet{kustowski2022suppressing} demonstrated that by using two-dimensional simulations, which are $10^3$ times faster to compute, a deep model could be trained on a relatively large dataset of simulations and, subsequently, fine-tuned on a small set of real-world data points. This fine-tuned model can significantly improve predictions compared to using real or simulation data points alone.

In the context of transfer learning, two key aspects can be explored: (1) Building representations that are more easily transferred; and (2) Developing a more sophisticated and effective transfer protocol. In scientific applications, these two aspects can potentially interact and complement each other. However, the multi-modal nature of scientific applications has not been fully addressed by existing methods, which often fail to explicitly model the inter-dependencies across modalities.

Multi-modal surrogate models often rely on a pretrained auto-encoding model to obtain a shared latent space that captures not only the variability of each modality but also their interactions. In the scientific domain, numerous efforts have been made to employ various auto-encoding architectures for this purpose. For instance, previous work utilized a Wasserstein Auto-Encoder based deep learning method, first training on simulation data and then fine-tuning on real data \citep{kustowski2022suppressing}. The model was initially trained to compress output scalars and images into a latent space and, then, reconstruct these outputs. Next, a surrogate model was trained to encode input scalars into the latent space. Finally, a single layer of the decoder (the one immediately following the latent space) was fine-tuned on real data to improve predictions on held-out validation data.

In contrast, our work adopts a fundamentally different approach, emphasizing the use of Transformer-based architectures. The recent development of vision transformers has showcased their effectiveness in learning unsupervised image representations \citep{dosovitskiy2021an}. We extend this approach to incorporate scalars alongside images, enabling the model to efficiently learn from multi-modal data. Our approach consistently outperforms prior work in predicting image and scalar values on held-out test data. By combining the new transformer-based architecture, masked auto-encoder pretraining, and a novel graph-based hyperparameter optimization, we achieve significant improvements in our few-shot learning scenario. 

Our key contributions include:
\begin{itemize}
\item Demonstrating the effectiveness 
of using Transformer-based neural networks to construct a multi-modal surrogate model for physical systems.
\item Introducing a novel graph-based hyper-parameter optimization technique to enable more robust few-shot transfer learning.
\item Showcasing the advantages of employing an MAE as a base model for few-shot fine-tuning, resulting in improved performance, validated through numerous experiments.
\end{itemize}

==> figs/sim_img_results.tex <==
\begin{figure}[!bt]
\centering
        \includegraphics[width=0.99\linewidth]{figs/mae_sim_improvements.pdf}
        \caption{Our models' predictions on ten random samples for the synthetic held-out test X-ray image after fine-tuning on the 9 synthetic training data, compared to the baseline. Pixels here represent energy outputs of the experimental implosion. White pixels are high energy, purple are lower energy, and black are no energy.  Zoom in to better see the results. The MSE for our method is lower than the baseline for the test predictions. While the image quality is not perfect, we find that our new model performs much better qualitatively as well as quantitatively than the baseline.
        }
        \label{fig:sim_image}
\end{figure}

==> figs/umap.tex <==
\begin{figure}[!bt]
\centering
        \includegraphics[width=0.30\linewidth]{figs/umaps/umap1.png}
        \includegraphics[width=0.30\linewidth]{figs/umaps/umap2.png}
        \includegraphics[width=0.30\linewidth]{figs/umaps/umap3.png}
        \caption{ Dimensionality reductions of the Neutron yield output embeddding to compare different tuned models. \textbf{(Left):} The UMAP of the pretrained model on the experiment data. \textbf{(Middle):} The UMAP of our optimally selected model. \textbf{(Right):} The UMAP of the lowest validation error overfit model.
        }
        \label{fig:umap}
\end{figure}

==> tables/tbl_masked_vs_pred.tex <==
\begin{table}[htbp]
\centering
\begin{tabular}{clccc}
Method     & Dataset   & Loss            & Scalar MSE  & Image MSE    \\ \hline
%\baseline & $\real$   & N/A             & 0.870       & $0.170$ \\
$\val$     & $\real$   & $L_{masked}$    & 0.643       & $0.164$ \\
$\graph$   & $\real$   & $L_{masked}$    & 0.566       & $0.157$ \\
$\val$     & $\real$   & $L_{pred}$      & 0.523       & $0.157$ \\
$\graph$   & $\real$   & $L_{pred}$      & \textbf{0.504}     & $\mathbf{0.149}$ \\ \hline
%\baseline & $\synth$  & N/A             & 6.851       & $0.079$ \\
$\val$     & $\synth$  & $L_{masked}$    & 5.076       & $0.031$  \\
$\graph$   & $\synth$  & $L_{masked}$    & \textbf{4.977}     & $\mathbf{0.030}$  \\
$\val$     & $\synth$  & $L_{pred}$      & 5.715       & $0.050$ \\
$\graph$   & $\synth$  & $L_{pred}$      & 5.583       & $0.039$  \\ \hline
\end{tabular}
\caption{Detailed results comparing the masked auto-encoder versus prediction only model, as well as using the smoothed graph validation error rate \mgraph versus the non-graph minimum validation error rate \mval. We find the interesting result that masking is useful for the $\synth$ dataset, but not for $\real$. Using the graph, however, is a consistent improvement.
\matt{This table should be 4 charts: scalars real, scalars synth, image real, image synth. I'm not quite sure how to show the 2x2 nature of the method x loss though. }
}
        \label{tbl:masked_vs_pred}
\end{table}

